Annihilating Dark Matter Search with 12 Years of Fermi LAT Data in Nearby Galaxy Clusters

Galaxy clusters are the largest virialised objects in the Universe, and as such, have a high dark matter (DM) concentration. This abundance of dark matter makes them promising targets for indirect DM searches. Here we report the details of a search, utilising almost 12~years of Fermi/LAT data, for gamma ray signatures from the pair annihilation of WIMP dark matter in the GeV energy band. From this, we present the constraints on the annihilation cross section for the bb-bar, W+W- and gamma-gamma channels, derived from the non-detection of a characteristic signal from five nearby high galactic latitude galaxy clusters (Centaurus, Coma, Virgo, Perseus and Fornax). We discuss the potential of a boost to the signal due the presence of substructures in the DM halos of selected objects, as well as the impact of uncertainties in DM profiles on the presented results. We assert that the obtained limits are, within a small factor, comparable to the best available limits of those based on Fermi/LAT observations of dwarf spheroidal galaxies.

==> referee_response1.tex <==
>1) The authors should make more clear what is new in this analysis. Other groups have used Fermi data in the direction of clusters and galaxy groups to constrain dark matter annihilation. Please review these studies, and make clear what is new about this paper. Obviously, more data is part of the distinction, but what else has been advanced in this submission?

We have elaborated these points further in the third paragraph of "results and discussion" section.

>2) As written in Eq 1, the quantities b_f and <sigma_f v> are redundant. I assume that the authors have not made this mistake in their calculations, but it should be corrected in its presentation.

In our analysis we have assumed a 100\% branching ratio to each considered annihilation state, thus negating the need for these values, as the referee correctly posits. However we have included them for posterity, and this is now explained in further detail in the text below equation 2.

>3) I find it strange to refer to Eq 3 as a "Zhao profile", when it is identical to a generalized NFW profile (which the authors later note).

Corrected. Please see text around equation 3 as well as the caption of table 1. We used name "Zhao profile" to keep consistency with CLUMPY code documentation, where generalized NFW profiles are named "ZHAO".

>4) The authors should make clear how some of their assumptions quantitatively impact their results. In particular, they make assumptions about the inner core of the profiles, about the minimum subhalo mass, and the spatial distribution of the subhalos. How do variations in these choices impact the resulting constraints?

We added a corresponding discussion, please see last two paragraphs section 2.4.

>5) In the conclusion, the authors argue that their results are complementary to those derived from gamma-ray studies of dwarf galaxies, citing a factor of ~2 uncertainties related to the dwarf J-factors. While I agree that this uncertainty does exist, similar (if not larger) uncertainties exist in the present analysis. This should be made more clear in the discussion.

Corrected, please see end of page 8.
